Learning Fair Scoring Functions: Bipartite Ranking under ROC-based Fairness Constraints

Many applications of AI involve scoring individuals using a learned function of their attributes. These predictive risk scores are then used to take decisions based on whether the score exceeds a certain threshold, which may vary depending on the context. The level of delegation granted to such systems in critical applications like credit lending and medical diagnosis will heavily depend on how questions of fairness can be answered. In this paper, we study fairness for the problem of learning scoring functions from binary labeled data, a classic learning task known as bipartite ranking. We argue that the functional nature of the ROC curve, the gold standard measure of ranking accuracy in this context, leads to several ways of formulating fairness constraints. We introduce general families of fairness definitions based on the AUC and on ROC curves, and show that our ROC-based constraints can be instantiated such that classifiers obtained by thresholding the scoring function satisfy classification fairness for a desired range of thresholds. We establish generalization bounds for scoring functions learned under such constraints, design practical learning algorithms and show the relevance our approach with numerical experiments on real and synthetic data.

==> parts/broader_impact.tex <==
% !TEX root = ../paper_supp.tex

\section*{Broader Impact}

Our work proposes different approaches to learn fair scoring functions.
The ideas presented here could be applied to a wide range of 
real-world applications
that have a scoring or ranking component.
% which arises whenever one allocates an unknown
% amount of finite resources to a set of most relevant instances.
% such as credit scoring, medical diagnosis, facial
% recognition or law enforcement.
In this context, it is well known that learning on historical data can induce
systemic discrimination of specific social groups. Our work proposes flexible
techniques to explicitly correct these biases, which is necessary to make
the deployment of
scoring algorithms more acceptable.
% Additionally, we provide mathematical evidence that those fairness requirements
% will be attained during deployment, in the form of generalization
% guarantees, which is under-explored yet crucial in most applications that
% involve scoring.

On the other hand, due the moral nature of fairness, there is a
lack of consensus on what makes a system fair,
see for instance the debate around  affirmative action.
In machine learning, this is reflected through the many
definitions of fairness introduced in recent years.
% , and motivated the unified
% and flexible nature of our approach.
In that context, our work is at risk of being exploited to advertise
a system as fair, even though it did not select the notion of fairness
that matches societal expectations or did not balance appropriately fairness
with ranking performance.
Our generalization guarantees further run the risk of being interpreted as a
mean to select fairness constraints, although they hold for all data
distributions and therefore cannot be expected to accurately predict
the observed trade-offs
between fairness and ranking performance for specific datasets. 

While we discussed the application of our methodology to real
data, it is clear that more applied research is needed to mitigate these
issues by proposing a
principled data-driven methodology for practitioners to select the appropriate
notion of fairness for their use-case, while also integrating the potential
costs in terms of ranking performance.
% This methodology could be backed by mathematical theory by relating
% specific characteristics of the distribution to potential fairness trade-offs,
% which would further prevent potential misuses of fairness constraints.

% \aurelien{Some ideas: take fairness angle to highlight the potential
% benefits, such as avoiding ML-based scoring that discriminate certain
% groups and ultimately a better societal acceptability of decision-making
% systems. For risks, we could mention the absence of societal agreement on what
% is the right notion of fairness, and this is even more the case for
% bipartite ranking as seen by the many fairness notions discussed in our work.
% A risk is then that our work is used to advertise a system as fair although it
% does not address the appropriate fairness challenges of the application. We
% have tried to discuss these issues and to illustrate on real data, but more
% practical work is needed to build a systematic methodology to choose the
% appropriate notion of fairness and the right trade-off with ranking
% performance based on the use-case}

